HealthLoopQA: A Context-Aware Question Answering Benchmark for Interpreting Wearable Monitoring Data in Diabetes Care

As medical wearables become integrated into daily chronic disease care, effectively interpreting longitudinal monitoring data is essential for patients and clinicians to understand health trends, detect safety-critical events, and make informed decisions. While large language models (LLMs) show promise for transforming this streaming physiological data into personalized health insights, evaluating their reasoning capability and analytical rigor in diverse monitoring tasks remains a fundamental challenge. Existing medical wearable question answering (QA) benchmarks primarily assess short-horizon classification or statistical summaries, largely ignoring the long-term patterns, therapeutic and behavioural contexts, and potential system failures inherent in real-world deployments. To address this, we introduce HealthLoopQA, a comprehensive diagnostic benchmark for evaluating LLM reasoning over continuous diabetes monitoring data. Grounded in a novel taxonomy of eleven atomic reasoning abilities, HealthLoopQA comprises 127 tasks and over 1,500 QA instances spanning process mining, anomaly detection, and prediction over 30-day horizons. To systematically evaluate safety awareness, we complement real-world datasets with a fault-injected simulation testbed modeling diverse device malfunctions and cyber-physical attacks to generate physiologically plausible hazard scenarios. Evaluating state-of-the-art LLMs across prompting and agentic frameworks reveals severe limitations in complex temporal pattern mining. Furthermore, we identify a broader phenomenon of In-context Laziness under long-context prompting, highlighting critical open challenges in deploying LLMs for rigorous long-horizon medical reasoning.

==> tables/atomic_reasoning.tex <==
\begin{table*}[hbt!]
\centering
\footnotesize
\begin{tabularx}{\linewidth}{XXXX}
\toprule
\textbf{Atomic Reasoning} & \textbf{Description} & \textbf{\textit{Example}} & \textbf{Purpose} \\
\midrule%\midrule

\textbf{Quantitative Calculation (QC)} & Execution of mathematical operations to derive a single numerical value. & \textit{mean, sum, standard deviation, maximum, minimum, counts, percentages.} & Forms the foundation of CGM statistical reasoning. \\
\midrule%\midrule

\textbf{Temporal Retrieval (TR)} & Locating and extracting temporal information such as timestamp and time window from the data. & \textit{(1) Retrieving the timestamp of a peak glucose reading. (2) Selecting the 3-hour post-meal window or the period after exercise of the glucose readings.} & Identifies when events occur and narrows reasoning to relevant temporal segments for analysis, essential for time-series reasoning. \\
\midrule%\midrule

\textbf{Event Filtering (EF)} & Identifying specific real-world events in the data. & \textit{Detecting exercise start/end times or meal timestamps.} & Anchors reasoning in contextual events for downstream analysis. \\
\midrule%\midrule

\textbf{Comparative Analysis (CA)} & Establishing relationships between two or more values or periods. & \textit{Comparing glucose variability in mornings vs.\ afternoons, or time-in-range across weeks.} & Enables contrastive reasoning built on QC, TR, DW, and EF. \\
\midrule%\midrule

\textbf{Anomaly Recognition (AR)} & Identifying physiologically implausible patterns or sensor artifacts. & \textit{Abrupt spikes/drops, flat-lines, abnormal insulin-glucose patterns.} & Ensures data integrity and highlights unusual events. \\
\midrule%\midrule

\textbf{Formatting Alignment (FA)} & Producing outputs in a structured and logically consistent format required by the task. & \textit{Constructing an interval from consecutive \texttt{NaN} readings, formatted as \texttt{\{"start": $t_1$, "end": $t_n$\}}.} & Ensures that answers follow the expected schema, enabling reliable downstream evaluation. \\
\midrule%\midrule

\textbf{Pattern Recognition (PR)} & Detecting recurring or unknown meaningful pattern within the glucose readings. & \textit{Daily rise–fall cycles, post-meal glucose curves, or repeated late-night hypoglycemia patterns.} & Captures higher-level behavioral or physiological regularities beyond individual data points. \\
\midrule%\midrule

\textbf{Predictive Forecasting (PF)} & Extrapolating from historical or current time-series patterns. & \textit{Predicting glucose 30 minutes ahead or forecasting overnight stability.} & Supports forward-looking reasoning and scenario anticipation. \\
\bottomrule
\end{tabularx}
\caption{Atomic reasoning types for that are essential for LLMs to answer the CGM questions, with descriptions, illustrative examples, and analytic purposes.}
\label{tab:atomic_reasoning}
\end{table*}


==> tables/data_statistics.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l c c c c}
\toprule
\textbf{Group} & \textbf{$N$} & \textbf{Regression\%} & \textbf{Classification\%} & \textbf{Event\%} \\
\midrule
Process Mining         & 900 & 69 & 24 & 7 \\
Anomaly Detection         & 1160 & 14 & 9 & 77 \\
Prediction         & 400 & 45 & 55 & 0 \\
\midrule
Descriptive & 740 & 63 & 33 & 3 \\
Memory      & 860 & 22 & 8 & 69 \\
Pattern     & 860 & 45 & 55 & 0 \\
\bottomrule
\end{tabular}
\caption{Dataset statistics across tasks and cognitive levels. We removed some questions that do not produce computable ground truth (e.g., the model consistently outputs \texttt{None} where a number are expected). $N$ denotes the final number of included questions.}
\label{tab:data-statistics}
\end{table}


==> tables/failure_types.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabularx}{\textwidth}{p{3cm}X}
\toprule
\textbf{Failure Type} & \textbf{Definition} \\
\midrule

\textbf{1. Reluctance to calculate} &
The models were reluctant to execute exact, precise programmatic operations (\textbf{QC}) over the 30-day dataset, as well as abandoning full-sequence anomaly scans (\textbf{AR}), suggesting that such operations are complex and thus less practicable. Instead, the models often estimate a value, partial results, return empty sets, or default to plausible heuristics. These failures highlight explicit limitations in both numerical accuracy and scaling to long sequences.
\\

\textbf{2. Temporal Misalignment} &
The models struggled in \textbf{TR}, for example: (i) correctly locating timestamps (e.g., day~7, 21:00), and (ii) correctly isolating predefined time windows (e.g., a 3-hour post-meal segment). Such failures reflect difficulties in temporal indexing and boundary alignment.
\\

\textbf{3. Unsupported Assumption} &
The models often defaulted to generating plausible but unsupported estimates, typically anchored in generic physiological priors (e.g., ``average glucose $\approx$ 140--150 mg/dL'') or context-based assumptions (e.g., inferring that glucose is unstable after a carb-heavy meal compared to a lighter one). While such heuristics occasionally succeed in trend or comparison tasks (\textbf{CA}), they consistently fail for queries requiring numerical precision.
\\

\textbf{4. Guessing over Abstaining} &
Even when the models explicitly acknowledged potential errors, they still produced assumption-based answers rather than expressing uncertainty and abstaining from producing an answer. This aligns with recent findings on LLM hallucinations \cite{kalai2025language}, which demonstrate that models often prefer guessing over admitting uncertainty, as training and evaluation procedures tend to reward the former.
\\

\textbf{5. Formatting Misalignment} &
The models sometimes failed to adhere to the required output format or granularity. Typical issues include returning plain text instead of JSON or merging multiple anomaly intervals into an overly broad span (\textbf{IC}). This failure type is relatively uncommon, and interval-formatting drift is often a downstream effect of temporal misalignment.
\\

\bottomrule
\end{tabularx}

\caption{
Reasoning failure types identified in HealthLoopQA.
}
\label{tab:failure_taxonomy}

\end{table*}

==> tables/reasoning_categories.tex <==

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l l}
\toprule
\textbf{Difficulty Level} & \textbf{Question IDs} \\
\midrule
Level 1: Computational Reasoning & 
pm\_0--2, pm\_4--13, pm\_15--19, pm\_38--45; \\
& ad\_1, ad\_2, ad\_25--27, ad\_31, ad\_32 \\
\midrule
Level 2: Retrieval and Mapping & 
pm\_3, pm\_14, pm\_20--22, pm\_24, pm\_26, pm\_28--34, pm\_36; \\
& ad\_3--24, ad\_28--30, ad\_33, ad\_35, ad\_36, ad\_37--40, \\
& ad\_42--54, ad\_57--64 \\
\midrule
Level 3: Comparative (Retrieval-based) & 
pm\_23, pm\_25, pm\_27, pm\_35, pm\_37; \\
& ad\_34, ad\_36 (alt. interpretation) \\
\midrule
Level 4: Predictive Forecasting & -- \\
\bottomrule
\end{tabular}
\caption{Categorization of \texttt{pm\_0--45} and \texttt{ad\_1--64} questions into reasoning difficulty levels.}
\label{tab:pm-ad-difficulty}
\end{table}


==> tables/reasoning_path.tex <==
\begin{table*}[hbt!]
\centering
\resizebox{0.99\linewidth}{!}{%
\begin{tabular}{l|l|l|c}
\toprule
\textbf{Hop Count} & \textbf{Reasoning Path(s)} & \textbf{Question IDs} & \textbf{Count} \\
\midrule\midrule
\textbf{1-hop} & QC & \textrm{pm\_0-2, pm\_9, pm\_41} & $6$ \\
\midrule\midrule
\multirow{2}{*}{\textbf{2-hop}} 
& QC $\rightarrow$ TR & \textrm{pm\_3, pm\_42, pm\_43} & $3$ \\
& DW $\rightarrow$ QC & \textrm{pm\_4-8, pm\_10-12, pm\_38-40} & $12$ \\
\midrule\midrule
\multirow{2}{*}{\textbf{3-hop}} 
& DW $\rightarrow$ QC $\rightarrow$ CA & \textrm{pm\_13, pm\_15-17} & $4$ \\
& TR $\rightarrow$ DW $\rightarrow$ QC & \textrm{pm\_14, pm\_44} & $2$ \\
\midrule\midrule
\multirow{3}{*}{\textbf{4-hop}} 
& TR $\rightarrow$ DW $\rightarrow$ QC $\rightarrow$ CA & \textrm{pm\_18-19, pm\_45} & $3$ \\
& TR $\rightarrow$ EF $\rightarrow$ DW $\rightarrow$ QC & \textrm{pm\_20-22, pm\_24-26, pm\_28-35} & $14$ \\
& EF $\rightarrow$ DW $\rightarrow$ QC $\rightarrow$ CA & \textrm{pm\_25, pm\_37} & $2$ \\
\midrule\midrule
\multirow{2}{*}{\textbf{5-hop}} 
& TR $\rightarrow$ EF $\rightarrow$ DW $\rightarrow$ QC $\rightarrow$ CA & \textrm{pm\_23, pm\_27} & $2$ \\
& TR $\rightarrow$ EF $\rightarrow$ DW $\rightarrow$ QC $\rightarrow$ TR & \textrm{pm\_36, pm\_22, pm\_32} & $3$ \\
\bottomrule
\end{tabular}}
\caption{Reasoning path taxonomy for CGM- and insulin-related questions, grouped by hop count. Higher hop counts indicate more cognitively demanding tasks that require chaining multiple reasoning steps.}
\label{tab:reasoning_paths}
\end{table*}


==> tables/results_table_test.tex <==

\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.12}

\newcommand{\ci}[2]{#1$_{\scriptscriptstyle #2}$}
\newcommand{\bestci}[2]{\textbf{#1}$_{\scriptscriptstyle \mathbf{ #2}}$}

\resizebox{\textwidth}{!}{
\begin{tabular}{llccc ccc ccccc c}
\toprule
\multirow{2}{*}{Model} &
\multirow{2}{*}{Method}
& \multicolumn{3}{c}{Time-series task}
& \multicolumn{3}{c}{Cognitive level}
& \multicolumn{6}{c}{Atomic skill}
& \multirow{2}{*}{Overall} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
\cmidrule(lr){9-14}
& & PM & AD & PD
& Desc. & Mem. & Patt.
& QC & TR & ER & CA & PR & PC
& \makecell{score$_{\scriptscriptstyle\mathrm{CI}_{95}}$} \\
\midrule

\multicolumn{14}{l}{\textit{Simulated dataset (127 tasks)}} \\
Gemini & Prompting
& \ci{67.4}{9.2} & \ci{21.2}{5.2} & \ci{62.3}{13.9}
& \ci{66.5}{14.9} & \ci{49.5}{10.2} & \ci{31.6}{7.6}
& \ci{59.1}{7.1} & \ci{43.2}{9.7} & \ci{56.0}{13.8} & \ci{40.8}{13.0} & \ci{44.4}{14.1} & \ci{22.4}{7.3}
& \ci{43.7}{6.0} \\
GPT & Agent
& \ci{88.3}{7.5} & \bestci{72.9}{7.4} & \bestci{74.6}{10.8}
& \ci{88.2}{10.0} & \bestci{91.4}{6.3} & \bestci{66.7}{7.2}
& \bestci{86.2}{5.1} & \bestci{86.3}{6.6} & \bestci{78.1}{11.5} & \bestci{87.2}{8.2} & \bestci{71.0}{9.9} & \bestci{63.6}{10.1}
& \bestci{78.5}{4.9} \\
Claude & Agent
& \bestci{92.4}{5.1} & \ci{70.6}{6.9} & \ci{64.8}{11.8}
& \bestci{91.6}{7.6} & \ci{89.5}{5.5} & \ci{64.0}{6.8}
& \ci{84.4}{5.0} & \ci{85.8}{5.8} &  \ci{74.8}{11.5} & \ci{83.8}{9.1} & \ci{64.8}{10.3} & \ci{63.4}{9.3} 
& \ci{77.1}{4.6} \\

\hdashline

\multicolumn{14}{l}{\textit{Simulated dataset (44 tasks)}} \\
Gemini & Prompting
& \ci{68.7}{9.1} & -- & \ci{62.4}{19.8}
& \ci{86.5}{8.9} & \ci{59.1}{11.9} & \ci{62.4}{19.8}
& \ci{67.4}{8.0} & \ci{59.2}{11.5} & \ci{59.3}{27.1} & \ci{57.3}{49.6} & \ci{46.5}{14.4}
& \ci{67.4}{8.0} \\
GPT & Agent
& \ci{88.2}{7.5} & -- & \bestci{78.0}{12.3}
& \ci{85.4}{15.1} & \ci{89.7}{9.0} & \bestci{78.0}{12.3}
& \ci{86.1}{6.4} & \ci{88.3}{9.1} & \bestci{79.0}{15.3} & \bestci{72.5}{31.7} & \bestci{86.1}{11.1}
& \ci{86.1}{6.4} \\
Claude & Agent
& \bestci{92.3}{5.1} & -- & \ci{66.8}{15.2}
& \bestci{92.5}{9.7} & \bestci{92.2}{6.4} & \ci{66.8}{15.2}
& \bestci{87.1}{5.6} & \bestci{90.7}{6.8} & \ci{66.3}{17.3} & \ci{65.7}{44.4} & \ci{85.5}{11.0}
& \bestci{87.1}{5.6} \\

\midrule

\multicolumn{14}{l}{\textit{Real-world dataset (44 tasks)}} \\
Gemini & Prompting
& \ci{62.5}{8.4} & -- & \ci{73.0}{15.6}
& \ci{79.0}{12.3} & \ci{59.8}{8.4} & \ci{73.0}{15.6}
& \ci{64.6}{7.3} & \ci{54.8}{9.0} & \ci{68.5}{20.4} & \ci{74.2}{43.0} & \ci{47.4}{15.1}
& \ci{64.6}{7.3} \\
GPT & Agent
& \bestci{88.7}{5.4} & -- & \bestci{75.7}{14.0}
& \ci{92.7}{9.9} & \bestci{86.6}{6.8} & \bestci{75.7}{14.0}
& \bestci{86.1}{5.2} & \bestci{83.4}{7.3} & \bestci{73.2}{17.0} & \bestci{83.9}{33.3} & \bestci{83.7}{10.8}
& \bestci{86.1}{5.2} \\
Claude & Agent
& \ci{87.4}{6.0} & -- & \ci{70.8}{13.0}
& \bestci{94.3}{9.7} & \ci{83.8}{7.6} & \ci{70.8}{13.0}
& \ci{84.1}{5.6} & \ci{82.3}{7.0} & \ci{68.7}{15.2} & \ci{77.5}{33.7} & \ci{79.7}{13.3}
& \ci{84.1}{5.6} \\
\bottomrule
\end{tabular}
}
\caption{
Overall performance by dataset portion, task type, cognitive level, and atomic skill. Entries report mean normalised scores scaled to 0--100, with subscripts indicating the half-width of the 95\% confidence interval. Bold values indicate the best score within each dataset portion and column. AD is unavailable for the real-world and matched simulated real-world portions.
}
\label{tab:quantitative-overall_test}
\end{table*}

==> tables/table_faults.tex <==
\begin{table*}[!htbp]
\centering
\caption{Final set of 17 fault patterns and 2 physiological hazards used in the simulation loop.}
\label{tab:faultpatterns}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{3cm} p{7.5cm} p{3.5cm} p{2cm}}
\toprule
\textbf{Failure Mode} & \textbf{Manipulation} & \textbf{Label} & \textbf{ad\_IDs} \\
\midrule
Missing signal &
Randomly replace $M$ consecutive points with NaN &
missing\_signal &
1, 2, 3, 12, 43 \\
\addlinespace

Positive spike readings &
BG spike $=$ value $+$ 60 mg/dL &
positive\_spike &
9, 10, 13, 16, 24, 36, 38, 55 \\
\addlinespace

Negative spike readings &
BG spike = value $-$ 60 mg/dL &
negative\_spike &
4, 9, 13, 14, 15, 33, 42, 54, 55 \\
\addlinespace

Repeated readings &
Repeat same value for $M > 6$ points &
repeated\_reading &
6, 7, 8, 11, 40, 42, 45 \\
\addlinespace

Negative biased readings &
BG $- 32$ mg/dL for $M$ points &
negative\_bias &
42, 47, 53, 60 \\
\addlinespace

Positive biased readings &
BG $+$ 32 mg/dL for $M$ points &
positive\_bias &
47, 53 \\
\addlinespace

Minimize readings &
BG forced to 70 mg/dL &
min\_reading &
42 \\
\addlinespace

Maximize readings &
BG forced to 180 mg/dL &
max\_reading &
50 \\
\addlinespace

Repeated episode &
Replay previous meal-driven BG segment &
repeated\_episode &
45 \\
\addlinespace

Zero readings &
BG = 0 &
zero\_reading &
8, 11, 42 \\
\addlinespace

False meal &
Controller registers a false meal event &
false\_meal &
44 \\
\addlinespace

False bolus &
Repeated bolus request without meal/exercise &
false\_bolus &
45, 46, 48, 49 \\
\addlinespace

Biased basal &
Basal rate $\pm$ 0.5 U/hr &
positive\_basal / negative\_basal &
46, 49 \\
\addlinespace

Maximize basal &
Set pump action $=$ 2 &
max\_basal &
48, 49, 52 \\
\addlinespace

Minimize basal &
Set pump action $=$ 0 &
min\_basal &
48, 49, 52, 58 \\
\addlinespace

Unknown stopped delivery &
Basal delivery forced to 0 while pump reports normal &
unknown\_stop &
58, 59, 62, 63 \\
\addlinespace

Unknown under delivery &
Basal reduced by 0.5 U/hr while pump reports normal &
unknown\_under &
60, 61, 64 \\
\addlinespace

Hypoglycemia \\(hazard) &
BG \textless{} 70 mg/dL &
hypoglycemia &
17, 18, 19, 20, 21, 22, 25, 26, 30, 31, 34, 35, 37 \\
\addlinespace

Hyperglycemia \\(hazard) &
BG \textgreater{} 180 mg/dL &
hyperglycemia &
21, 23, 27, 28, 29, 31, 32, 34, 37 \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/table_qa.tex <==
% \begin{table*}[t]
% \centering
% %\resizebox{.95\columnwidth}{!}{
% \begin{tabular}{l|l|l|l}
%     authblk & babel & cjk & dvips \\
%     epsf & epsfig & euler & float \\
%     fullpage & geometry & graphics & hyperref \\
%     layout & linespread & lmodern & maltepaper \\
%     navigator & pdfcomment & pgfplots & psfig \\
%     pstricks & t1enc & titlesec & tocbind \\
%     ulem
% \end{tabular}
% \caption{LaTeX style packages that must not be used.}
% \label{table1}
% \end{table*}

\begin{table*}[!t]
\centering
\small
\caption{Prototype questions designed for each time series task in HealthLoopQA.}
\label{tab:prototype_questions}
\begin{tabular}{p{1.5cm}p{5.5cm}p{5.5cm}}
\toprule
\textbf{Time-series Task}&  \textbf{Prototype}&\textbf{Question Examples} \\
\midrule
\textbf{Process Mining} & 
 &\\
\midrule
\textbf{Anomaly Detection} & 
 \textbf{Faulty Patterns}: missing signal, spike/repeated/bias/minimise/maximise/zero readings, repeated episode,  unknown stop/under delivery, false meal, false bolus, bias/minimise/maximise basal, comparison/indicated anomalies&- Was there a data dropout over the last weekend (28th and 29th)? \newline - Were there any overnight periods with unusually stable CGM readings? \newline - My glucose dropped fast after lunch today. Has this happened before, and if so, when?\\
\cmidrule(lr){2-3}
 & \textbf{Malfunctions}: loss of sensitivity to  glucose, miscalibration, CGM sensor error, communication loss, pressure-induced sensor attenuation, unphysiological spikes, lowered local glucose concentration, stop delivery, under delivery&- When might the CGM sensor have been dislodged? \newline - Were there any time intervals when my sensor readings showed signs of possible miscalibration? \newline - Is there any period that may indicate pressure-induced sensor attenuation?\\
 \cmidrule(lr){2-3}
 & \textbf{Cyberattacks}: availability attack, process-aware attacks, replay attacks, personalised insulin dose manipulation attack, bias injection attacks, unauthorised remote control, command manipulation attack, saturation-based sensor spoofing attack, false data injection attack, malicious pump driver&- Were there any periods with suspiciously repeated BG readings? \newline - Were there any periods indicating unauthorised access or manipulation of my insulin delivery? \\
  \cmidrule(lr){2-3}
 & \textbf{Hazards}: hypoglycemia, hyperglycemia, hazard recovery&- During which time intervals at night did hypoglycemia episodes occur? \newline - How long did it generally take to reach the target range after a prolonged hyperglycemia episode?\\
\midrule
\textbf{Prediction} & 
\textbf{Patient behaviour }: insulin usage, meal impact on body &- Which exercise is better for me to bring down blood sugar tomorrow - cycling or running? \newline - Will I need a correction insulin dose in the next 2 hours? &
\bottomrule
\end{tabular}
\end{table*}
